Scalable Finite Adaptability via Polyhedral Partition and Learning

We study finite adaptability for decision-making under uncertainty, where a finite set of candidate decisions is prepared in advance and a response is selected after uncertainty is realized. Despite advances in exact formulations, scalability remains challenging due to combinatorial decision assignments and the joint optimization of uncertainty set partitions and associated decisions. We develop a framework that explicitly parameterizes polyhedral partitions, enabling direct optimization of partition boundaries and associated decisions. We establish convergence of such polyhedral policies to the fully adjustable benchmark under general risk measures, including a rate of $O(K^{-\alpha/n})$ under uniform $\alpha$-H\"older continuity, where $K$ is the number of regions and $n$ is the uncertainty dimension. Exploiting the explicit polyhedral structure, we derive two exact reformulations for robust finite adaptability, one based on master--subproblem cut generation and the other on piecewise dualization, and extend the framework to stochastic programming. To improve scalability, we introduce an approximate-learn-parallel algorithm that integrates partition learning with parallel regional optimization while preserving robustness. Computational experiments on classical robust and stochastic testbeds demonstrate scalability to larger instances and competitive policy performance.

==> Figures/figure_style.tex <==
% Shared typography for Figures 1 and 2. Both are resized to the same
% manuscript width, so an identical source canvas also gives identical
% printed font sizes. Keep these definitions local to each figure group.
\newcommand{\faFigureFont}{\fontsize{10}{11}\selectfont}%
\newcommand{\faFigureDetailFont}{\fontsize{9}{10}\selectfont}%
\newcommand{\faNormalizeFigureWidth}{%
  \coordinate (faFigureTop) at (current bounding box.north);
  \coordinate (faFigureBottom) at (current bounding box.south);
  \pgfresetboundingbox
  \path[use as bounding box] ([xshift=-8.5cm]faFigureBottom)
    rectangle ([xshift=8.5cm]faFigureTop);
}%

